A General Framework for Robust G-Invariance in G-Equivariant Networks

We introduce a general method for achieving robust group-invariance in group-equivariant convolutional neural networks ($G$-CNNs), which we call the $G$-triple-correlation ($G$-TC) layer. The approach leverages the theory of the triple-correlation on groups, which is the unique, lowest-degree polynomial invariant map that is also complete. Many commonly used invariant maps--such as the max--are incomplete: they remove both group and signal structure. A complete invariant, by contrast, removes only the variation due to the actions of the group, while preserving all information about the structure of the signal. The completeness of the triple correlation endows the $G$-TC layer with strong robustness, which can be observed in its resistance to invariance-based adversarial attacks. In addition, we observe that it yields measurable improvements in classification accuracy over standard Max $G$-Pooling in $G$-CNN architectures. We provide a general and efficient implementation of the method for any discretized group, which requires only a table defining the group's product structure. We demonstrate the benefits of this method for $G$-CNNs defined on both commutative and non-commutative groups--$SO(2)$, $O(2)$, $SO(3)$, and $O(3)$ (discretized as the cyclic $C8$, dihedral $D16$, chiral octahedral $O$ and full octahedral $O_h$ groups)--acting on $\mathbb{R}^2$ and $\mathbb{R}^3$ on both $G$-MNIST and $G$-ModelNet10 datasets.

==> sections/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}


==> sections/scratch.tex <==
% These computations have not been included in the main paper.

\section{Equivariance of the $G$-Convolution}\label{sec:g-conv}


The $G$-convolution is \textit{equivariant} to the action of the group $G$ on the domain of the signal $\signal$~\cite{cohen2016group}. This means that any action $\action_h$ on the domain of $\signal$ results in a corresponding action $\action'_h$ on the output of the convolutional layer. Specifically, for a filter $\filter $, the equivariance property is:
\begin{equation}
    \filter * \action_{h}[\signal] = \action'_{h}[\filter * \signal], \qquad \text{for all ${h} \in G$,}
\end{equation}
where $\action_h$ and $\action'_h$ represent the actions of the same group element $h$ on $\signal$ and $\filter * \signal$ respectively.



\begin{proof}
Consider a signal $\signal: \domain \rightarrow \mathbb{R}^c$ and a filter $\filter: \domain \rightarrow \mathbb{R}^c$ defined on a domain $\domain$ and codomain $\mathbb{R}^c$, with $c$ the number of channels.

For transformations $h, g \in G$, we have:
\begin{align*}
    \filter * \action_{h}[\signal](g)
        &= \int_{u \in \domain} 
            \filter(\action_{g^{-1}}(u)) \action_{h}[\signal](u) du \\
        &= \int_{u \in \domain} 
            \filter(\action_{g^{-1}}(u))\signal( \action_{h^{-1}}(u)) du \\
        &= \int_{u' \in \domain} 
            \filter(\action_{g^{-1}}(\action_{h}(u')))\signal(u') du' 
            \qquad 
            \text{($u' =  \action_{h^{-1}}(u)$, i.e., $u = \action_{h}(u')$)} \\
        &= \int_{u \in \domain} 
            \filter(\action_{g^{-1}h}(u))\signal(u) du \\
        &= \int_{u \in \domain} 
            \filter(\action_{(h^{-1}g)^{-1}}(u))\signal(u) du \\
        &= \int_{u \in \domain} 
            \action_{(h^{-1}g)}[\filter](u)\signal(u) du \\
        &=\action'_{h}[\filter * \signal](g)
\end{align*}
where the action $L'$ uses $h$ to act on the domain $G$ of the output signal  $[\filter * \signal]$ by left multiplication with $h^{-1}$.
\end{proof}

This property applies for the $G$-convolutions of the first layer and of the next layers.

\section{Example of Triple Correlation on $C_4$}

In this appendix, we work out the computations of the TC for the group $C_4$ shown in the explanatory Figure of the main text.

The group is $G = C_4$ and the first input real signal is $\Theta$ defined as:

\begin{equation}
    \Theta(0) = 0, \quad \Theta(1) = -1, \quad \Theta(2) = 1, \quad \Theta(3) = 2.
\end{equation}

We compute the elements of the triple correlation.

First the $(0, 0)$ diagonal element.
\scriptsize
\begin{align*}
    \tau_\Theta(0, 0)
    = \sum_{g \in G} \Theta(g)^3
    = 0^3 + (-1)^3 + 1^3 + 2^3
    = 8
\end{align*}

\normalsize
Then we populate the first line of the TC and add the values of the TC for the symmetric elements.
\scriptsize
\begin{align*}
\tau_\Theta(0, 1)
    &= \sum_{g \in G} \Theta(g)^2 \Theta(g+1)\\
    &= \Theta(0)^2 \Theta(0+1)
    + \Theta(1)^2 \Theta(1+1)
    + \Theta(2)^2 \Theta(2+1)
    + \Theta(3)^2 \Theta(3+1) \\
    &= \Theta(0)^2 \Theta(1)
    + \Theta(1)^2 \Theta(2)
    + \Theta(2)^2 \Theta(3)
    + \Theta(3)^2 \Theta(0) \\
    &= 0 + (-1)^2.1 + 1^2.2+0\\
    &=3 \\
    &=\tau_\Theta(1, 0)\\
    &=\tau_\Theta(0^{-1}, 1.0^{-1}) = \tau_\Theta(0, 1) \\
    &=\tau_\Theta(1^{-1}, 0.1^{-1}) = \tau_\Theta(3, 3)\\
\tau_\Theta(0, 2)
    &= \sum_{g \in G} \Theta(g)^2 \Theta(g+2)\\
    &= \Theta(0)^2 \Theta(0+2)
    + \Theta(1)^2 \Theta(1+2)
    + \Theta(2)^2 \Theta(2+2)
    + \Theta(3)^2 \Theta(3+2) \\
    &= \Theta(0)^2 \Theta(2)
    + \Theta(1)^2 \Theta(3)
    + \Theta(2)^2 \Theta(0)
    + \Theta(3)^2 \Theta(1) \\
    &= 0 + (-1)^2.2 + 0 + 2^2.(-1)\\
    &= -2 \\
    &=\tau_\Theta(2, 0)\\
    &=\tau_\Theta(0^{-1}, 2.0^{-1}) = \tau_\Theta(0, 2) \\
    &=\tau_\Theta(2^{-1}, 0.2^{-1}) = \tau_\Theta(2, 2)\\
\tau_\Theta(0, 3)
    &= \sum_{g \in G} \Theta(g)^2 \Theta(g+3)\\
    &= \Theta(0)^2 \Theta(0+3)
    + \Theta(1)^2 \Theta(1+3)
    + \Theta(2)^2 \Theta(2+3)
    + \Theta(3)^2 \Theta(3+3) \\
    &= \Theta(0)^2 \Theta(3)
    + \Theta(1)^2 \Theta(0)
    + \Theta(2)^2 \Theta(1)
    + \Theta(3)^2 \Theta(2) \\
    &= 0 + 0 + 1^2.(-1) + 2^2.1\\
    &= 3 \\
    &=\tau_\Theta(3, 0)\\
    &=\tau_\Theta(0^{-1}, 3.0^{-1}) = \tau_\Theta(0, 3) \\
    &=\tau_\Theta(3^{-1}, 0.3^{-1}) = \tau_\Theta(1, 1).
\end{align*}

\normalsize
Then, we populate the second line of the TC.
\scriptsize
\begin{align*}
\tau_\Theta(1, 2)
    &= \sum_{g \in G} \Theta(g) \Theta(g+1)\Theta(g+2)\\
    &= \Theta(0) \Theta(0+1)\Theta(0+2)
    + \Theta(1) \Theta(1+1)\Theta(1+2)
    + \Theta(2) \Theta(2+1)\Theta(2+2)
    + \Theta(3) \Theta(3+1)\Theta(3+2) \\
    &= \Theta(0) \Theta(1)\Theta(2)
    + \Theta(1) \Theta(2)\Theta(3)
    + \Theta(2) \Theta(3)\Theta(0)
    + \Theta(3) \Theta(0)\Theta(1) \\
    &= 0
    + -1.1.2
    + 0
    + 0\\
    &=-2\\
    &=\tau_\Theta(2, 1)\\
    &=\tau_\Theta(1^{-1}, 2+1^{-1}) = \tau_\Theta(3, 2+3)=\tau_\Theta(3, 1) =\tau_\Theta(1, 3) \\
    &=\tau_\Theta(2^{-1}, 1+2^{-1}) = \tau_\Theta(2, 1+2)=\tau_\Theta(2, 3) =\tau_\Theta(3, 2).
\end{align*}
\normalsize
\section{Example of Triple Correlation on $\mathbb{Z}_2 \times \mathbb{Z}_2$}

In this appendix, we work out the computations of the TC for the group $\mathbb{Z}_2 \times \mathbb{Z}_2$ shown in the explanatory Figure of the main text.

The group is $G = \mathbb{Z}_2 \times \mathbb{Z}_2 $ and the first input real signal is $\Theta$ defined as:
\begin{equation}
    \Theta(00) = 2, \quad \Theta(01) = 0, \quad \Theta(10) = 1, \quad \Theta(11) = 1.
\end{equation}

We compute the elements of the triple correlation.

\scriptsize
\begin{align*}
    \tau_\Theta(00, 00) 
    &= \sum_{g \in G} \Theta(g)^3 
    = 8+0+1+1 
    = 10 \\
    \tau_\Theta(00, 01) 
    &=\sum_{g \in G} \Theta(g)^2\Theta(g \cdot 01) \\
    &= \Theta(00)^2\Theta(01) 
        + \Theta(01)^2\Theta(01\cdot 01)
        + \Theta(10)^2\Theta(10\cdot 01)
        + \Theta(11)^2\Theta(11\cdot 01)\\
    &= \Theta(00)^2\Theta(01) 
        + \Theta(01)^2\Theta(00)
        + \Theta(10)^2\Theta(11)
        + \Theta(11)^2\Theta(10)\\
    &= 2^2 .0 +0^2.2+1^2.1+1^2.1
    = 2 \\
    \tau_\Theta(00, 10) 
    &=\sum_{g \in G} \Theta(g)^2\Theta(g \cdot 10) \\
    &= \Theta(00)^2\Theta(10) 
        + \Theta(01)^2\Theta(01\cdot 10)
        + \Theta(10)^2\Theta(10\cdot 10)
        + \Theta(11)^2\Theta(11\cdot 10)\\
    &= \Theta(00)^2\Theta(10) 
        + \Theta(01)^2\Theta(11)
        + \Theta(10)^2\Theta(00)
        + \Theta(11)^2\Theta(01)\\
    &= 2^2 .1 +0^2.1+1^2.2+1^2.0
    = 3 \\ 
    \tau_\Theta(00, 11) 
    &= \sum_{g \in G} \Theta(g)^2\Theta(g \cdot 11) \\
    &= \Theta(00)^2\Theta(11) 
        + \Theta(01)^2\Theta(01\cdot 11)
        + \Theta(10)^2\Theta(10\cdot 11)
        + \Theta(11)^2\Theta(11\cdot 11)\\
    &= \Theta(00)^2\Theta(11) 
        + \Theta(01)^2\Theta(10)
        + \Theta(10)^2\Theta(01)
        + \Theta(11)^2\Theta(00)\\
    &= 2^2 .1 +0^2.1+1^2.0+1^2.2 = 6 \\
    % Don't compute these: Get the diagonal elements with symmetry
    % \tau_\Theta(01, 01) 
    % &= \sum_{g \in G} \Theta(g)\Theta(g \cdot 01)^2 \\ 
    % &= \Theta(00)\Theta(00 \cdot 01)^2 
    % + \Theta(01)\Theta(01 \cdot 01)^2 
    % + \Theta(10)\Theta(10 \cdot 01)^2 
    % + \Theta(11)\Theta(11 \cdot 01)^2 \\
    % &= \Theta(00)\Theta(01)^2 
    % + \Theta(01)\Theta(00)^2 
    % + \Theta(10)\Theta(11)^2 
    % + \Theta(11)\Theta(10)^2 \\
    % &= 2.0^2 
    % + 0.2^2 
    % + 1.1^2 
    % + 1.1^2 = 2 \\
    % \tau_\Theta(10, 10) 
    % &= \sum_{g \in G} \Theta(g)\Theta(g \cdot 10)^2 \\ 
    % &= \Theta(00)\Theta(00 \cdot 10)^2 
    % + \Theta(01)\Theta(01 \cdot 10)^2 
    % + \Theta(10)\Theta(10 \cdot 10)^2 
    % + \Theta(11)\Theta(11 \cdot 10)^2 \\
    % &= \Theta(00)\Theta(10)^2 
    % + \Theta(01)\Theta(11)^2 
    % + \Theta(10)\Theta(00)^2 
    % + \Theta(11)\Theta(01)^2 \\
    % &= 2.1^2 
    % + 0.1^2 
    % + 1.2^2 
    % + 1.0^2 = 6 \\
    % \tau_\Theta(11, 11) 
    % &= \sum_{g \in G} \Theta(g)\Theta(g \cdot 11)^2 \\ 
    % &= \Theta(00)\Theta(00 \cdot 11)^2 
    % + \Theta(01)\Theta(01 \cdot 11)^2 
    % + \Theta(10)\Theta(10 \cdot 11)^2 
    % + \Theta(11)\Theta(11 \cdot 11)^2 \\
    % &= \Theta(00)\Theta(11)^2 
    % + \Theta(01)\Theta(10)^2 
    % + \Theta(10)\Theta(01)^2 
    % + \Theta(11)\Theta(00)^2 \\
    % &= 2.1^2 
    % + 0.1^2 
    % + 1.0^2 
    % + 1.2^2 = 6 \\
    \tau_\Theta(01, 10) 
    &= \sum_{g \in G} \Theta(g)\Theta(g \cdot 01) \Theta(g \cdot 10) \\
    &= \Theta(00)\Theta(00 \cdot 01) \Theta(00 \cdot 10)
    + \Theta(01)\Theta(01 \cdot 01) \Theta(01 \cdot 10)
    + \Theta(10)\Theta(10 \cdot 01) \Theta(10 \cdot 10)
    + \Theta(11)\Theta(11 \cdot 01) \Theta(11 \cdot 10)\\
    &=\Theta(00)\Theta( 01) \Theta(10)
    + \Theta(01)\Theta(00) \Theta(11)
    + \Theta(10)\Theta(11) \Theta(00)
    + \Theta(11)\Theta(10) \Theta(01)\\
    &=2.0.1
    + 0.2.1
    + 1.1.2
    + 1.1.0\\
    &=2 \\
    \tau_\Theta(11, 10) 
    &= \sum_{g \in G} \Theta(g)\Theta(g \cdot 11) \Theta(g \cdot 10) \\
    &= \Theta(00)\Theta(00 \cdot 11) \Theta(00 \cdot 10)
    + \Theta(01)\Theta(01 \cdot 11) \Theta(01 \cdot 10)
    + \Theta(10)\Theta(10 \cdot 11) \Theta(10 \cdot 10)
    + \Theta(11)\Theta(11 \cdot 11) \Theta(11 \cdot 10)\\
    &=\Theta(00)\Theta(11) \Theta(10)
    + \Theta(01)\Theta(10) \Theta(11)
    + \Theta(10)\Theta(01) \Theta(00)
    + \Theta(11)\Theta(00) \Theta(01)\\
    &=2.1.1
    + 0.1.1
    + 1.0.2
    + 1.2.0\\
    &=2
\end{align*}

\normalsize

The second input real signal is $\Theta'$ defined as:
\begin{equation}
    \Theta'(00) = 0, \quad \Theta'(01) = 1, \quad \Theta'(10) = 1, \quad \Theta'(11) = 2.
\end{equation}

We compute the triple correlation for $\Theta'$

\scriptsize 
\begin{align*}
    \tau_\Theta'(00, 00) 
    &= \sum_{g \in G} \Theta'(g)^3 
    = 0+1+1+8 
    = 10 \\
    \tau_\Theta'(00, 01) 
    &=\sum_{g \in G} \Theta'(g)^2\Theta'(g \cdot 01) \\
    &= \Theta'(00)^2\Theta'(01) 
        + \Theta'(01)^2\Theta'(01\cdot 01)
        + \Theta'(10)^2\Theta'(10\cdot 01)
        + \Theta'(11)^2\Theta'(11\cdot 01)\\
    &= \Theta'(00)^2\Theta'(01) 
        + \Theta'(01)^2\Theta'(00)
        + \Theta'(10)^2\Theta'(11)
        + \Theta'(11)^2\Theta'(10)\\
    &= 0^2 .1 +1^2.0+1^2.2+2^2.1
    = 6 \\
    \tau_\Theta'(00, 10) 
    &=\sum_{g \in G} \Theta'(g)^2\Theta'(g \cdot 10) \\
    &= \Theta'(00)^2\Theta'(10) 
        + \Theta'(01)^2\Theta'(01\cdot 10)
        + \Theta'(10)^2\Theta'(10\cdot 10)
        + \Theta'(11)^2\Theta'(11\cdot 10)\\
    &= \Theta'(00)^2\Theta'(10) 
        + \Theta'(01)^2\Theta'(11)
        + \Theta'(10)^2\Theta'(00)
        + \Theta'(11)^2\Theta'(01)\\
    &= 2^2 .1 +1^2.2+1^2.0+2^2.1
    = 14 \\ 
    \tau_\Theta'(00, 11) 
    &= \sum_{g \in G} \Theta'(g)^2\Theta'(g \cdot 11) \\
    &= \Theta'(00)^2\Theta'(11) 
        + \Theta'(01)^2\Theta'(01\cdot 11)
        + \Theta'(10)^2\Theta'(10\cdot 11)
        + \Theta'(11)^2\Theta'(11\cdot 11)\\
    &= \Theta'(00)^2\Theta'(11) 
        + \Theta'(01)^2\Theta'(10)
        + \Theta'(10)^2\Theta'(01)
        + \Theta'(11)^2\Theta'(00)\\
    &= 0^2 .2 +1^2.1+1^2.1+2^2.0 = 2 \\
    \tau_\Theta'(01, 10) 
    &= \sum_{g \in G} \Theta'(g)\Theta'(g \cdot 01) \Theta'(g \cdot 10) \\
    &= \Theta'(00)\Theta'(00 \cdot 01) \Theta'(00 \cdot 10)
    + \Theta'(01)\Theta'(01 \cdot 01) \Theta'(01 \cdot 10)
    + \Theta'(10)\Theta'(10 \cdot 01) \Theta'(10 \cdot 10)
    + \Theta'(11)\Theta'(11 \cdot 01) \Theta'(11 \cdot 10)\\
    &=\Theta'(00)\Theta'( 01) \Theta'(10)
    + \Theta'(01)\Theta'(00) \Theta'(11)
    + \Theta'(10)\Theta'(11) \Theta'(00)
    + \Theta'(11)\Theta'(10) \Theta'(01)\\
    &=0.1.1
    + 1.0.1
    + 1.2.0
    + 2.1.1\\
    &=2 \\
    \tau_\Theta'(11, 10) 
    &= \sum_{g \in G} \Theta'(g)\Theta'(g \cdot 11) \Theta'(g \cdot 10) \\
    &= \Theta'(00)\Theta'(00 \cdot 11) \Theta'(00 \cdot 10)
    + \Theta'(01)\Theta'(01 \cdot 11) \Theta'(01 \cdot 10)
    + \Theta'(10)\Theta'(10 \cdot 11) \Theta'(10 \cdot 10)
    + \Theta'(11)\Theta'(11 \cdot 11) \Theta'(11 \cdot 10)\\
    &=\Theta'(00)\Theta'(11) \Theta'(10)
    + \Theta'(01)\Theta'(10) \Theta'(11)
    + \Theta'(10)\Theta'(01) \Theta'(00)
    + \Theta'(11)\Theta'(00) \Theta'(01)\\
    &=0.2.1
    + 1.1.2
    + 1.1.0
    + 1.0.1\\
    &=2
\end{align*}
\normalsize
\newpage

\section{Algorithmic Reduction of the Triple Correlation}\label{app:reduction}

\subsection{Direct Approach}

In the ``direct approach'', we ask:\\

\textit{which TC coefficients do we need to reconstruct the original signal?}\\

We note that we do not care about whether the reconstruction is computationally expensive, as we will not implement it in practice. We are only interested in knowing the minimal number of TC coefficients that fully represent $f$.

We consider a simple example on $Z_n$

Consider a real signal defined on $Z_n$: $f(0), ..., f(n-1)$. Try to design an algorithm to recover that signal from some values of the triple correlation.


We compute some quantities related to the TC that could be helpful:
\begin{equation}
    a(0, 0) = \sum_{x = 0}^{n-1} f(x)^3
\end{equation}


\begin{equation}
   \sum_{x'=0}^{n-1} a(0, x') =  \sum_{x'=0}^{n-1} \sum_{x = 0}^{n-1} f(x)^2f(x-x')
\end{equation}


\subsection{Bispectrum Approach}

In the ``bispectrum approach'', we ask:\\

\textit{which TC coefficients do we need to reconstruct the first column of the bispectrum?}\\

If we can reconstruct the first column of the bispectrum, then we can reconstruct the signal. Again, we do not care whether the reconstruction itself is computationally expensive.

We write the definition of the bispectrum (first column) and look at the triple correlation coefficients involved.

We have:
\begin{align*}
    \beta(f)_{k_1, k_2}
        &=
    \frac{1}{n^3}\sum_{x_1 \in Z_n} \sum_{x_2 \in Z_n} 
    T(f)(x_1, x_2)\left[
                \rho_1(x_1)^{\dagger} \otimes \rho_2(x_2)^{\dagger}
            \right]\\
    &=
    \frac{1}{n^3}\sum_{x_1 \in Z_n} \sum_{x_2 \in Z_n} 
    \left(\sum_{x \in Z_n} 
       f^*(x) 
       f\left(x + x_1\right) f\left(x+ x_2\right)\right)
            \left[
                \rho_1(x_1)^{\dagger} \otimes \rho_2(x_2)^{\dagger}
            \right]
\end{align*}
where each representation $\rho_j$ is associated with and integer $k_j$ such that: $\rho_1(x') = \exp(-i\frac{2k_1\pi x'}{n})$ and $\rho_2(x') = \exp(-i\frac{2k_2\pi x'}{n})$ for any $x' \in Z_n$.

We are only interested in the first column of the bispectrum. Thus, we set $k_1 = 0$ or equivalently $\rho_1(x') = 1$ for all $x' \in Z_n$:
\begin{align*}
    \beta(f)_{0, k_2}
        &=
    \sum_{x_1 \in Z_n} \sum_{x_2 \in Z_n} 
    T(f)(x_1, x_2)\left[
                1 \otimes \rho_2(x_2)^{\dagger}
            \right]\\
    &=
    \sum_{x_1 \in Z_n} \sum_{x_2 \in Z_n} 
    \left(\sum_{x \in Z_n} 
       f^*(x) 
       f\left(x + x_1\right) f\left(x+ x_2\right)\right)
            \left[
                1\otimes \rho_2(x_2)^{\dagger}
            \right]\\
    % &=
    % \sum_{x_1 \in Z_n} 
    % \left(\sum_{x \in Z_n} 
    %    f^*(x) 
    %    f\left(x + x_1\right) \sum_{x_2 \in Z_n} f\left(x+ x_2\right) \rho_2(x_2)^{\dagger}\right).
\end{align*}

At this stage, we see that even if we set $k_1=0$, we still need all the $x_1, x_2$ terms of the triple correlation.

We can continue the computations, to see if we can get rid of $x_1$.
\begin{align*}
    \beta(f)_{0, k_2}
    &=
   \sum_{x_2 \in Z_n} \left(\sum_{x \in Z_n} f^*(x) f\left(x+ x_2\right) \rho_2(x_2)^{\dagger}
      \sum_{x_1 \in Z_n}  f\left(x + x_1\right) \right)\\
          &=
    \sum_{x_2 \in Z_n} \left(\sum_{x \in Z_n}  f^*(x) f\left(x+ x_2\right) \rho_2(x_2)^{\dagger}
      \sum_{x_1' \in Z_n}  f\left(x_1'\right) \right) \quad \text{(change of variable $x'_1 = x + x_1$)}\\
          &=
    \sum_{x_1' \in Z_n}\sum_{x_2 \in Z_n}\left(\sum_{x \in Z_n}  f^*(x) f\left(x+ x_2\right) f\left(x_1'\right)\right) \rho_2(x_2)^{\dagger},
\end{align*}

Unfortunately, this does not make a simpler TC term appear.

We try another version of the computations, to see if we can get rid of $x_2$.
\begin{align*}
    \beta(f)_{0, k_2}
    &=
    \sum_{x_1 \in Z_n} 
    \left(\sum_{x \in Z_n} 
       f^*(x) 
       f\left(x + x_1\right) \rho_2(-x).\hat{f}_{k_2}\right) \quad \text{(equivariance of Fourier transform)}\\
    &=
   \hat{f}_{k_2}
    \left(\sum_{x \in Z_n} 
       f^*(x)  \rho_2(-x)\sum_{x_1 \in Z_n} 
       f\left(x + x_1\right) \right) \\
    &=
    \hat{f}_{k_2}
    \left(\sum_{x \in Z_n} 
       f^*(x)  \rho_2(-x)\sum_{x_1' \in Z_n} 
       f\left(x_1'\right) \right) \quad \text{change of variable}\\
    &=
    \hat{f}_{k_2}
    \left(\sum_{x \in Z_n} 
       f(x)  \rho_2(x)^\dagger\right)^*\left(\sum_{x_1' \in Z_n} 
       f\left(x_1'\right) \right)\\
    &=
    \hat{f}_{k_2}
    \hat{f}_{k_2}^*\left(\sum_{x_1' \in Z_n} 
       f\left(x_1'\right) \right)\\
    &=
    \hat{f}_{k_2}
    \hat{f}_{k_2}^*\hat{f}_{0} 
\end{align*}
We recovered the formula of the bispectrum, but this does not help figuring which TC coefficients we need: we find that we need only some fourier coefficients, as expected.

\paragraph{From previous meeting} Define the triple correlation of a single group element:

\begin{align}
\label{eq:tc0}
    a(0, g) = \int_{g^{\prime}} f(g^{\prime})^2 f(g^{\prime} g) dg^{\prime} \\ 
\end{align}

Recall the bispectrum on a single irrep:

\begin{align}
    A(0, \rho) &= \hat{f}_0 \hat{f}_{\rho} \hat{f}_{\rho}^{\dagger} \\
    &= \int_{g^{\prime}} f(g^{\prime}) dg^{\prime} \int_g f(g) \rho(g)^{\dagger} dg \int_g f(g)^{\dagger} \rho(g) dg
\end{align}

We take the group Fourier transform of \ref{eq:tc0} to obtain:

\begin{align}
    \mathcal{F}_{\rho}(a) &= \int_{g} a(0, g) \rho_{g}^{\dagger} dg \\ 
    &= \int_{g} \int_{g_2} f(g_2)^2 f(g_2 g) dg_2 \rho_{g}^{\dagger} dg \\ 
    &= \int_{g} \int_{g_2} f(g_2) \rho_g f(g_2) \rho_g^{\dagger} f(g_2 g) dg_2 \rho_{g}^{\dagger} dg \\
    &= \int_{g_2} f(g_2) f(g_2) dg_2  \int_{g} f(g_2 g)\rho_g  \rho_g^{\dagger}\rho_{g}^{\dagger} dg \\
    &= \int_{g_2} f(g_2) f(g_2) dg_2  \int_{g'} f(g')\rho_{g_2}\rho_{g'} dg' \\
&= \int_{g_2} f(g_2) f(g_2) dg_2  \rho_{g_2} \left(\int_{g'} f(g')\rho_{g'} dg'\right) \\
&= \int_{g'} f(g')f(g')  \rho_{g'} dg'  \left(\int_{g} f(g)\rho_{g} dg\right) 
\end{align}
if $\rho_{g'} = \rho$ was independent of $g'$, we could conclude, because we could say that the function $f$ and $\rho f$ are linearly dependant, such that they are colinear vectors in the space of functions. We could then apply the equality case of Cauchy-Schwarz to get:
\begin{align}
\mathcal{F}_{\rho}(a) 
    &= \int_{g'} f(g')f(g')  \rho dg'  \left(\int_{g} f(g)\rho_{g} dg\right) \\
    &= \sqrt{\int_{g'} f(g')^2dg'} \sqrt{\int_{g'} \rho^2 f(g')^2dg'}  \left(\int_{g} f(g)\rho_{g} dg\right) 
\end{align}
which is close to what we want, but not even what we want.


% \begin{proof}
% Consider a signal $\signal$ and a filter $\phi_k$. For a transformation ${\tilde{g}} \in G$, we have:
% \begin{align*}
%     \filter * \action_{\tilde{g}}[\signal](g)
%         &= \int_{u \in \domain} 
%             \filter(\action_{g^{-1}}(u)) \action_{\tilde{g}}[\signal](u) du \\
%         &= \int_{u \in \domain} 
%             \filter(\action_{g^{-1}}(u))\signal( \action_{\tilde{g}}(u)) du \\
%         &= \int_{u' \in \domain} 
%             \filter(\action_{g^{-1}}(\action_{\tilde{g}^{-1}}(u')))\signal(u') du' 
%             \qquad 
%             \text{($u' =  \action_{\tilde{g}}(u)$ i.e. $u =  \action_{\tilde{g}^{-1}}(u)$)} \\
%         &= \int_{u \in \domain} 
%             \filter(\action_{g^{-1}\tilde{g}^{-1}}(u))\signal(u) du \\
%         &= \int_{u \in \domain} 
%             \filter(\action_{(\tilde{g}g)^{-1}}(u))\signal(u) du \\
%         &=\action'_{\tilde{g}}[\filter * \signal](g)
% \end{align*}
% where the action $L'$ uses $\tilde{g}$ to act on the domain $G$ of the output signal  $[\filter * \signal]$ by left multiplication.

% TODO: What property allows to say that $g \domain = \domain$? Homogeneity implies that fact to be true, but we can find a more relaxed property and define the convolution on more general spaces.
% \end{proof}
